Guided Image Feature Matching using Feature Spatial Order

Image feature matching plays a vital role in many computer vision tasks. Although many image feature detection and matching techniques have been proposed over the past few decades, it is still time-consuming to match feature points in two images, especially for images with a large number of detected features. Feature spatial order can estimate the probability that a pair of features is correct. Since it is a completely independent concept from epipolar geometry, it can be used to complement epipolar geometry in guiding feature match in a target region so as to improve matching efficiency. In this paper, we integrate the concept of feature spatial order into a progressive matching framework. We use some of the initially matched features to build a computational model of feature spatial order and employs it to calculates the possible spatial range of subsequent feature matches, thus filtering out unnecessary feature matches. We also integrate it with epipolar geometry to further improve matching efficiency and accuracy. Since the spatial order of feature points is affected by image rotation, we propose a suitable image alignment method from the fundamental matrix of epipolar geometry to remove the effect of image rotation. To verify the feasibility of the proposed method, we conduct a series of experiments, including a standard benchmark dataset, self-generated simulated images, and real images. The results demonstrate that our proposed method is significantly more efficient and has more accurate feature matching than the traditional method.

==> config/acm.tex <==
%=============================%
%   DO NOT MODIFY THIS FILE   %
%=============================%

\ifx\varDocClass\undefined
\def \varDocClass{acmart}
\fi

\ifx\varKeyvals\undefined
\def \varKeyvals{sigconf}
\fi

\def\insertAuthors{}

\makeatletter
\newcommand{\addAuthor}[2]{
	\g@addto@macro\insertAuthors{\author{#1}}
	\@for\varRef:={#2}\do{
		\expandafter\g@addto@macro\expandafter\insertAuthors\expandafter{\expandafter\getInst\expandafter{\varRef}}
	}
	\g@addto@macro\insertAuthors{ }
}

\newcommand{\addInst}[2]{\expandafter\gdef\csname my@inst@#1\endcsname{#2}}
\newcommand{\getInst}[1]{\csname my@inst@#1\endcsname}

\newcounter{instId}
\newcommand{\addInstitution}[4]{
	\stepcounter{instId}
	\addInst{\theinstId}{
		\affiliation{
			\institution{#1}
			\city{#2}
			\country{#3}
		}
		\email{#4}
	}
}
\makeatother

\newcommand{\addAbstract}[1]{\def\varAbstract{#1}}
\newcommand{\addTitle}[1]{\def\varTitle{#1}}
\newcommand{\addKeywords}[1]{\def\varKeywords{#1}}
\def\insertRunningHeads{}
\newcommand{\setRunningHeads}[1]{
	\def\insertRunningHeads{\renewcommand{\shortauthors}{#1}}
}

\newcommand{\insertTopmatter}{
	\title{\varTitle}
	\insertAuthors
	\insertRunningHeads
	\begin{abstract}
		\varAbstract
	\end{abstract}
	\keywords{\varKeywords}
	\maketitle
}

\newcommand{\setBibStyle}{\bibliographystyle{bibliography/ACM-Reference-Format}}

%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
	\providecommand\BibTeX{{%
			\normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information.  This information is sent to you
%% when you complete the rights form.  These commands have SAMPLE
%% values in them; it is your responsibility as an author to replace
%% the commands and values with those provided to you when you
%% complete the rights form.
%\setcopyright{acmcopyright}
%\copyrightyear{2018}
%\acmYear{2018}
%\acmDOI{10.1145/1122445.1122456}

%% These commands are for a PROCEEDINGS abstract or paper.
%\acmConference[Woodstock '18]{Woodstock '18: ACM Symposium on Neural
%	Gaze Detection}{June 03--05, 2018}{Woodstock, NY}
%\acmBooktitle{Woodstock '18: ACM Symposium on Neural Gaze Detection,
%	June 03--05, 2018, Woodstock, NY}
%\acmPrice{15.00}
%\acmISBN{978-1-4503-XXXX-X/18/06}
